ARMOR: High-Performance Semi-Structured Pruning via Adaptive Matrix Factorization

Large language models (LLMs) present significant deployment challenges due to their immense computational and memory requirements. While semi-structured pruning, particularly 2:4 sparsity, offers a path to practical hardware acceleration, existing methods often incur substantial performance degradation. To bridge this gap, we introduce ARMOR: (Adaptive Representation with Matrix-factORization), a novel one-shot post-training pruning algorithm. Instead of directly pruning weights, ARMOR factorizes each weight matrix into a 2:4 sparse core wrapped by two low-overhead, block diagonal matrices. These wrappers act as efficient pre and post-transformation error correctors, offering greater flexibility to preserve model quality compared to conventional 2:4 pruning techniques. The sparse core and block diagonal wrappers are chosen through a block coordinate descent algorithm that minimizes a layer-wise proxy loss. We theoretically prove this optimization is guaranteed to converge to a solution with a proxy loss less than or equal to state-of-the-art pruning algorithms. Experiments on Llama (Touvron et al., 2023; Dubey et al., 2024) and Qwen (Yang et al., 2025) model families demonstrate that ARMOR consistently and significantly outperforms state-of-the-art 2:4 pruning methods across a wide range of downstream tasks and perplexity evaluations. ARMOR achieves this superior performance while retaining the inference speedups and substantial memory usage reductions of 2:4 pruning, establishing a more effective trade-off between model compression and task accuracy

==> Tabels/Ablations/Correlation.tex <==
\begin{table}[h!]
\begin{center}
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.2}
\small
\begin{tabular}{l | c | c }
\toprule
& \multicolumn{2}{c|}{Correlation Coefficient $(\uparrow)$} \\
Model & Wikitext-2 & C4 \\
\hline
Llama-2 7B & 0.991 & 0.990 \\
Llama-2 13B & 0.991 & 0.991 \\
Llama-3 8B & 0.994 & 0.995 \\
\bottomrule
\end{tabular}
\caption{\green{Pearson correlation coefficient between normalized change in global average proxy Loss and perplexity. Proxy loss and perplexity were logged every 1250 iterations, out of a total of 10,000 iterations of optimization. A block size of 128 was used}}
\label{tab:Correlation}
\end{center}
\end{table}

==> Tabels/Ablations/Normalization.tex <==
\begin{table}[h!]
\begin{center}
\setlength{\tabcolsep}{6.5pt} 
\renewcommand{\arraystretch}{1.2}
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{l | c | c |}
\toprule
Dataset & Wikitext 2 $(\downarrow)$ & C4 $(\downarrow)$\\
\hline
RedPajama-Data-1T & 7.59 & 9.89\\
\gr SlimPajama-627B & 7.68 & 9.88\\
\hline
\end{tabular}
\caption{\red{TODO}}
\label{tab:Qwen25Results}
\end{center}
\end{table}

==> Tabels/Ablations/ProxyLoss.tex <==
\begin{table}[h!]
\begin{center}
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.2}
\small
\begin{tabular}{l | c | c }
\toprule
Method & Wikitext-2 $(\downarrow)$ & C4 $(\downarrow)$ \\
\hline
\method + Wanda & 7.65 & \textbf{9.88} \\
\gr \method + NoWag & \textbf{7.59} & \textbf{9.88} \\
\bottomrule
\end{tabular}
\caption{\green{Wikitext 2 and C4 perplexity of \method pruned Llama-2 7B using different proxy losses. A block size of 128 was used, and optimization was ran for 5000 iterations.}}
\label{tab:ProxyAblation}
\end{center}
\end{table}

==> Tabels/Ablations/Rsquare.tex <==
\begin{table}[h!]
\begin{center}
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.2}
\small
\begin{tabular}{l | c | c }
\toprule
& \multicolumn{2}{c|}{Log-Log $R^2$ $(\uparrow)$} \\
Model & Wikitext 2 & C4  \\
\hline
Llama-2 7B & 0.99 & 0.99 \\
Llama-2 13B & 0.97 & 0.96 \\
Llama-3 8B & 0.99 & 0.98 \\
\bottomrule
\end{tabular}
\caption{\green{Linear regression $R^2$ fit for log-log Wikitext 2 and C4 perplexity vs iterations for Llama-2 7B, 13B, and Llama-3 8B. The \method optimization algorithm was run for 10,000 iterations, with perplexity being logged every 1,250 iterations. A block size of 128 was used}}
\label{tab:r2_fit}
\end{center}
\end{table}

==> Tabels/InferenceLayerwise.tex <==
\begin{table}[htb!]
    \centering
    \small
    \begin{tabular}{l | c c c c|}
        \toprule
         & 2.5-7B & 2.5-14B & 2.5-32B & 2.5-72B \\
         \hline
        Dense & - &  9.04 ms & - & - \\
        2:4 & - &  4.85 ms (\textbf{1.86}x) & - & - \\
        \method & - & 5.77 ms (\textbf{1.57}x) & - & - \\
        \bottomrule
    \end{tabular}
    \caption{Bench-marked matrix-vector multiplication on the gate projection layers of Qwen 2.5 models of varying sizes (7B, 14B, 32B, and 72B), compared between the original dense matrices, naive 2:4 pruned matrices, and \method factorization}
    \label{tab:speedMatMul}
\end{table}
